Direct Consistency Optimization for Robust Customization of Text-to-Image Diffusion Models

Text-to-image (T2I) diffusion models, when fine-tuned on a few personal images, can generate visuals with a high degree of consistency. However, such fine-tuned models are not robust; they often fail to compose with concepts of pretrained model or other fine-tuned models. To address this, we propose a novel fine-tuning objective, dubbed Direct Consistency Optimization, which controls the deviation between fine-tuning and pretrained models to retain the pretrained knowledge during fine-tuning. Through extensive experiments on subject and style customization, we demonstrate that our method positions itself on a superior Pareto frontier between subject (or style) consistency and image-text alignment over all previous baselines; it not only outperforms regular fine-tuning objective in image-text alignment, but also shows higher fidelity to the reference images than the method that fine-tunes with additional prior dataset. More importantly, the models fine-tuned with our method can be merged without interference, allowing us to generate custom subjects in a custom style by composing separately customized subject and style models. Notably, we show that our approach achieves better prompt fidelity and subject fidelity than those post-optimized for merging regular fine-tuned models.

==> figures/main/main_qual_momsgen.tex <==
\begin{figure*}[t]
    \small\centering
    \includegraphics[width=0.96\textwidth]{resources/main/qual_momsgen.pdf}
    \vspace{-5pt}
    \caption{
    \textbf{Compositional generation of {my subject in my style}.}
    We show generated examples of \emph{my subject in my style} with various actions or visual attributes given by text prompts by merging the customized models with DCO loss (\emph{i.e.}, DCO Merge).
    % fine-tuned with DCO the subject and style.
    % We merge independently trained subject and style personalized models with our method (\emph{i.e.}, DCO Merge). 
    Best viewed in color, zoomed in on monitor.}
    \label{fig:myobjectmystyle_gen}
    % \vspace{-5pt}
\end{figure*}

==> figures/main/main_quant.tex <==
\begin{figure*}[t]
    \centering\small
    \begin{subfigure}[t]{0.31\textwidth}
        \includegraphics[width=\linewidth]{resources/main_subject.pdf}
        \vspace{-10pt}
        \caption{Subject customization}
        \label{fig:quant_subject}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.31\textwidth}
        \centering\small
        \includegraphics[width=\linewidth]{resources/graphs/quan_style.pdf}
        \vspace{-10pt}
        \caption{Style customization}
        \label{fig:quant_style}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.31\textwidth}
        \centering\small
        \includegraphics[width=\linewidth]{resources/main_pref2.pdf}
        \vspace{-10pt}
        \caption{User study}
    \label{fig:user_study}
    \end{subfigure}
    % \vspace{-5pt}
    \caption{\textbf{Quantitative results.} We compare DCO (ours) with DreamBooth (DB) and DreamBooth with prior preservation (DB+p.p.) on \ref{fig:quant_subject} subject customization, \ref{fig:quant_style} style customization by evaluating image-text similarity and image similarity score. We provide user study results in \ref{fig:user_study}. 
    % conduct ablation studies on (a) comprehensive caption, (b) $\beta$, and (c) noise distance between pretrained model and fine-tuned model. 
    }
    \label{fig:main_quant}
    \vspace{-20pt}
\end{figure*}

==> figures/main/main_table.tex <==
\begin{table}[t]
\begin{minipage}[t]{0.56\textwidth}
\centering\small
\setlength\tabcolsep{2.5pt} 
\caption{
\textbf{Quantitative results.}
We compare DCO (ours) with DreamBooth (DB) and DB with prior preservation loss (DB+p.p.) on subject personalization under evaluation on each subject recontextualization and stylization. 
We report subject similarity ({\tt Subject}) using DINOv2~\citep{oquab2023dinov2} and image-text similarity ({\tt Text}) using SigLIP~\citep{zhai2023sigmoid}. *Note that we use harmonic mean since this is a multi-objective problem.
}
\label{tab:subject_table}
\begin{tabular}{@{}l|ccc | ccc @{}}
\toprule
 &
  \multicolumn{3}{c}{Recontextualization} &
  \multicolumn{3}{c}{Stylization} \\
  \cmidrule{2-4}\cmidrule{5-7}
   & DB & DB+p.p. & DCO  & DB & DB+p.p. & DCO \\
\midrule
% {\tt Subject} & 0.630 & 0.508 & 0.628 && 0.638 & 0.491 & 0.613 \\
% {\tt Text}  & 0.754 & 0.816 & 0.794 && 0.468 & 0.632 & 0.567 \\
{\tt Subject} & 0.630 & 0.532 & 0.628 & 0.638 & 0.424 & 0.613 \\
{\tt Text}  & 0.754 & 0.865 & 0.794 & 0.468 & 0.851 & 0.567 \\
% {\tt Subject} & 0.630 & 0.532 & 0.600 & 0.638 & 0.424 & 0.587 \\
% {\tt Text}  & 0.754 & 0.865 & 0.831 & 0.468 & 0.851 & 0.667 \\
\midrule
{\tt Mean*} & 0.686 & 0.659 & 0.701 & 0.540 & 0.567 & 0.589 \\
\bottomrule
\end{tabular}%
\end{minipage}
\hfill
\begin{minipage}[t]{0.42\textwidth}\label{tab:user_eval}
\centering\small
\setlength\tabcolsep{2.5pt}
\caption{
{\bf User evaluation.} 
We asked the users to select better one given two images generated by DCO vs. baselines (DB and DB+p.p.) for each question: 1) subject fidelity, 2) image-text alignment, and 3) image quality. We report the percentage of judgements in favor of DCO over baselines.}

% \begin{tabular}{@{}l ccc@{}}
% \toprule
%   Method & Img Sim. & IT Sim.  & Img quality \\
% \midrule
% DCO vs. DB & 57.2\% & 70.8\% & 69.0\% \\
% DCO vs. DB+p.p. & 81.2\% & 57.9\% & 63.8\% \\
% \bottomrule
% \end{tabular}

\begin{tabular}{@{}l cc@{}}
\toprule
  Win rate & vs. DB & vs. DB+p.p. \\
\midrule
{\tt Subject fidelity} & 55.1 \% & 81.9 \% \\
{\tt Prompt fidelity}  & 72.7 \% & 58.0 \% \\
{\tt Image quality} & 70.6 \% & 63.0 \% \\
\bottomrule
\end{tabular}

\end{minipage}
\label{tab:main}
\end{table}


==> figures/main/quan_moms.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Quantitative results of {my subject in my style} generation.} We report subject, style, and image-text similarity scores of arithmetic merge of DB subject and style models (DB Merge), ZipLoRA of DB models (DB ZipLoRA), and arithmetic merge of DCO models (DCO Merge). 
}\label{tab:quan_moms}
% \vspace{-5pt}
\centering\small
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{lccc}
\toprule
%      & DB Merge & DB ZipLoRA & DCO Merge \\ 
% \midrule
% Subject Similarity & 0.386   & 0.406     & {\bf 0.462}    \\
% Style Similarity    & {\bf 0.672}   & 0.662     & 0.651    \\
% Image-Text Similarity      & 0.430   & 0.729     & {\bf 0.773}    \\
     & Sub. Sim. & Style Sim. & I-T Sim. \\
\midrule
DB Merge & 0.386 & 0.672 & 0.430 \\
DB ZipLoRA & 0.406 & 0.662 & 0.729 \\
DCO Merge (ours) & {\bf 0.462} & 0.651 & {\bf 0.773} \\ 
\bottomrule
\end{tabular}
% \vspace{-20pt}
% }
\end{table}



==> figures/main/quantitative_style.tex <==
\begin{figure}[t]
    \small\centering
    \includegraphics[width=0.9\columnwidth]{resources/graphs/quan_style.pdf}
    \vspace{-5pt}
    \caption{
    \textbf{Quantitative results in style personalization.} 
    We plot image similarity and image-text similarity for style customization experiment for DreamBooth (DB) and DCO (ours). We plot the scores from reward guidance sampling (dots and dotted lines), and conventional classifier-free guidance sampling (diamond). See Sec.~\ref{sec:exp_style} for more details.
    }
    \label{fig:quan_style}
    \vspace{-10pt}
\end{figure}
